EcoRank: Budget-Constrained Text Re-ranking Using Large Language Models

Large Language Models (LLMs) have achieved state-of-the-art performance in text re-ranking. This process includes queries and candidate passages in the prompts, utilizing pointwise, listwise, and pairwise prompting strategies. A limitation of these ranking strategies with LLMs is their cost: the process can become expensive due to API charges, which are based on the number of input and output tokens. We study how to maximize the re-ranking performance given a budget, by navigating the vast search spaces of prompt choices, LLM APIs, and budget splits. We propose a suite of budget-constrained methods to perform text re-ranking using a set of LLM APIs. Our most efficient method, called EcoRank, is a two-layered pipeline that jointly optimizes decisions regarding budget allocation across prompt strategies and LLM APIs. Our experimental results on four popular QA and passage reranking datasets show that EcoRank outperforms other budget-aware supervised and unsupervised baselines.

==> Sections/intro_draft.tex <==
\section{Introduction}\label{sec:intro}
Text re-ranking focus on ranking $k$ source documents given a specific query and is crucial for providing the relevant retrieved context to downstream tasks. It serves either as a standalone task or as an intermediate step  for questions answering tasks in a retrival augmented setting, where the answer is generated from the top $k$ relevant passages. Traditional ranking methods includes BM25 [CITE] and neural methods like DPR [CITE,also others]. Recently, large language models (LLMs) such as GPT-4~\citep{openai2023gpt} 
have demonstrated dominant performance in text re-ranking [CITE]. 

However, utilizing LLMs often comes at a cost: the process can be quite expensive due to closed-source LLMs charging by token numbers. This expense escalates in text re-ranking, as it involves inputting substantial text, proportional to the number of passages to re-rank.

have been proven to be effective in a wide variety of language tasks such as question answering, code generation, text classification etc. Recently, we have seen an influx of LLMs with varied sizes, which can either be hosted offline with expensive hardware requirements such as GPUs or be accessed via APIs hosted by commercial organizations with a certain cost. LLMs such as openAI's or GPT-3~\citep{brown2020language} have shown impressive performances, even surpassing supervised models for various natural language tasks. Unfortunately, using LLMs for a high-throughput task like text-reranking can be quite expensive as we need to input a lot of text to the LLMs, proportional to the number of passages that need to be re-ranked.
For example, the cost of re-ranking 500 passages for a single query could be minimum of 5 USD using GPT-4~\citep{openaiprice}. For businesses which deal with thousands of queries in a single day, the cost may be way above their \textit{budget}. The cost typically depends on three components: 1) The length of the prompt or input 2) The length of the tokens generated, and sometimes 3) a fixed cost per query.

There are many companies (OpenAI, TextSynth, AI21, Cohere, Replicate etc.) that offer LLMs as a service via APIs with varied costs. While larger sized LLMs with higher costs typically means stronger performance, they may not necessarily work the best when working within a budget. Larger sized models may also not necessarily work better than smaller models for certain tasks. Further, for text re-ranking, prompts can be designed in a variety of ways, some prompts may be effective but costly, while some may work only with a certain sized LLM. Thus, achieving the best performance from text re-ranking using LLM APIs within a given budget is quite challenging.

Previous works that use LLM-based approaches for text re-ranking either use 1) Pointwise prompts~\citep{sachan2022improving}: which inputs a single passage per query per request and outputs calibrated prediction probabilities before sorting. \textit{Generation-only} LLMs (like GPT-3, GPT-4) are not supported for these prompts as they do not generate probabilities or scores of output tokens, or 2) Listwise prompts~\citep{sun2023chatgpt, ma2023zero}: which inputs mutiple passages per query per request as lists and asks LLMs to output the lists in an order. These prompts are rather difficult for medium-sized LLMs as they have difficulties parsing the prompt and generate correct output~\citep{qin2023large}, thus only costly APIs such as GPT-4 are applicable, or 3) Pairwise prompts~\citep{qin2023large}: which inputs pairs of passages per query per request and uses a sliding window to sort the top-k passages. \textit{However, all these works do not consider the cost of LLMs while doing text re-ranking.}. This is especially critical, as some approaches like pairwise and listwise are quite expensive as the prompt size is large. Using GPT-4, to re-rank 500 passages per query, pointwise approaches cost around 5 USD and pairwise cost about $10 \cdot k$ USD for top-k passages.

There has been work on cost-aware use of LLM ~\citep{chen2023frugalgpt, yue2023large, vsakota2023fly}. These works have proposed the idea of \textit{LLM Cascading} (i.e. combining multiple LLMs) to reduce cost but have the following limitations: 
\textit{(1)} None of their proposed approaches are applicable for \textit{text re-ranking} task, like \textit{answer sampling} strategy from MoT~\citep{yue2023large} requires multiple sample of answers which is only applicable to \textit{reasoning} tasks. 
\textit{(2)} They require a fine-tuned model (with training data) to score the generation quality of LLMs~\citep{chen2023frugalgpt, vsakota2023fly}.
\textit{(3)} Although they focus on reducing the cost of API calls, they do not consider an overall \textit{budget} as a constraint.

In this paper, we propose a suite of budget-constrained methods to perform text reranking using a set of LLM APIs. 
The input is a pre-ranked list of $N$ texts (i.e. passages) based on query $q$, a budget $\beta$, and a set of LLM APIs. The output is a re-ranked list of the $N$ texts. 
To the best of our knowledge, this is the first paper to consider the cost of LLMs for the \textit{text re-ranking} task.
Our most efficient method, which we refer as {\oursystem}, is a budget-constrained LLM-based text reranking pipeline, that jointly optimizes several objectives: 1) which prompt designs to deploy, 2) which LLM API to call, and 3) how to split budget between multiple prompts and LLMs.
Optimizing all these decisions jointly is challenging for the following reasons. 
(a) The provided budget may not even be enough to input all input texts once to the LLM API. The developed method must be able to optimize for the top-few (e.g. top-1) text.
(b) Different LLM APIs may have different strengths and limitations.
(c) We do not have any training data on how to best split the budget.
(d) There is an exponential number of combinations of prompt designs and API selections.

% An interesting observation is that {\oursystem} achieves the best performance even if there was no budget constraint, which proves the efficacy of our pipeline. 

We first show different text re-ranking prompt designs to solve the re-ranking task within a budget. We then investigate different available LLM APIs and their costs to employ such prompts. Finally, we propose a novel two-layer pipeline {\oursystem}, which first re-ranks the initially ranked passages (e.g. ranked using BM25) using \textit{pointwise relevance filtering} on a \textit{high-accuracy} (and thus \textit{expensive}) LLM API spending a fraction of our budget. This first level of re-ranking filters the irrelevant passages down the list so that we spend the rest of our budget on relatively relevant passages. In the second layer, we spend the rest of our budget using a \textit{less accurate} (thus \textit{cheaper}) LLM API to further re-rank the passages using \textit{pairwise ranking prompting}. 
%This ensures the relative ordering among the relevant passages. {\oursystem} is able to overcome the weaknesses of each individual prompt design and at the same time optimizes the cost by intelligently picking which passages to spend budget on. It is completely zero-shot, requires no training data and is able to produce state-of-the-art ranking performance.

We evaluate various single or hybrid (combining more than one) prompt designs for the text re-ranking problem, for various budgets and APIs on two popular QA benchmark datasets: Natural Questions (NQ)~\citep{kwiatkowski2019natural} and Web Questions (WebQ)~\citep{berant2013semantic}. Our most efficient method {\oursystem} achieves a gain of 14\% on MRR and R@1 ranking accuracy than other budget-aware prompt designs.
%We show that, given a budget constraint most prompt designs fail to utilize their full potential and {\oursystem} obtains a gain of 14\% on top-50 re-ranking accuracy. 
In summary we claim the following contributions.
\begin{itemize}
    \item We introduce the problem of budget-constrained text re-ranking that considers the cost of various LLM APIs.
    \item We propose and compare various ranking prompt designs and API choices in a budget-constrained scenario for text re-ranking.
    \item We further propose a novel two-layer cascading pipeline {\oursystem} which optimizes the budget usage.
    %by intelligently making a decision on the input to spend budget on which achieves state-of-the-art performance.
    \item We extensively evaluate and compare various prompt designs and API choices on two datasets. We make our code available to the research community~\footnote{a sample footnote}.
\end{itemize}

The rest of the paper is organized as follows. We define the scope and problem statement in Section~\ref{sec:problem}. We explain in details all the ranking prompt designs in Section~\ref{sec:ranking_algo} and most efficient approach {\oursystem} in Section~\ref{sec:our_system}. We present the results of our experimental evaluation in Section~\ref{sec:evaluation}. We discuss the related work in Section~\ref{sec:related} and finally conclude in Section~\ref{sec:conclusion}.



==> Tables/unlimited.tex <==
\begin{table}
%\scriptsize
\small
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
 \multirow{2}{*}{Setting}& \multicolumn{3}{c|}{NQ} & \multicolumn{3}{c}{WQ}\\
         &  \multicolumn{1}{c}{MRR}&  \multicolumn{1}{c}{R@1}& \multicolumn{1}{c|}{R@10} & \multicolumn{1}{c}{MRR}&  \multicolumn{1}{c}{R@1}& \multicolumn{1}{c}{R@10}\\
         \hline
         BM25&  32.49&  22.10& 54.45 & 29.69& 18.89&52.16\\
         Binary&  46.87&  37.36&  64.37& 42.09& 31.54&61.76\\
         Likert&  39.49&  28.25&  63.07& 39.81& 28.44&62.05\\
         UPR&  26.88&  16.48&  48.25& 28.41& 18.15&51.13\\
         PRP&  52.80&  45.34&  \textbf{66.53}& 48.07& 40.55&\textbf{63.09}\\
 {\oursystem}& \textbf{52.98}& \textbf{46.01}& 65.18& \textbf{48.71}& \textbf{40.99}&62.64\\
 \hline
    \end{tabular}
    \caption{Prompt designs with no budget constrain for top-50 passages}
\label{tab:unlimited}
    
\end{table}
